An Objective Improvement Approach to Solving Discounted Payoff Games

While discounted payoff games and classic games that reduce to them, like parity and mean-payoff games, are symmetric, their solutions are not. We have taken a fresh view on the constraints that optimal solutions need to satisfy, and devised a novel way to converge to them, which is entirely symmetric. It also challenges the gospel that methods for solving payoff games are either based on strategy improvement or on value iteration.

==> eptcsdata.tex <==
\providecommand{\firstpage}{203}
\providecommand{\publicationstatus}{A. Achilleos and D. Della Monica (Eds.): Fourteenth\\
International Symposium on Games, Automata, Logics,\\
and Formal Verification (GandALF 2023).\\
EPTCS 390, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.390.13}{10.4204/EPTCS.390.13}}

